RAIRS: Optimizing Redundant Assignment and List Layout for IVF-Based ANN Search

IVF is one of the most widely used ANNS (Approximate Nearest Neighbors Search) methods in vector databases. The idea of redundant assignment is to assign a data vector to more than one IVF lists for reducing the chance of missing true neighbors in IVF search. However, the naive strategy, which selects the second IVF list based on the distance between a data vector and the list centroids, performs poorly. Previous work focuses only on the inner product distance, while there is no optimized list selection study for the most popular Euclidean space. Moreover, the IVF search may access the same vector in more than one lists, resulting in redundant distance computation and decreasing query throughput. In this paper, we present RAIRS to address the above two challenges. For the challenge of the list selection, we propose an optimized AIR metric for the Euclidean space. AIR takes not only distances but also directions into consideration in order to support queries that are closer to the data vector but father away from the first chosen list's centroid. For the challenge of redundant distance computation, we propose SEIL, an optimized list layout that exploits shared cells to reduce repeated distance computations for IVF search. Our experimental results using representative real-world data sets show that RAIRS out-performs existing redundant assignment solutions and achieves up to 1.33x improvement over the best-performing IVF method, IVF-PQ Fast Scan with refinement.

==> cover.tex <==
\section*{Revision Letter}

We thank the meta-reviewer and all the reviewers for their valuable
comments and suggestions. 
%
We have revised the paper to address the raised issues according to
the revision plan.

In the following, we use (page number, section, paragraph) to indicate
the location of the revised contents, where the paper number refers to
the main paper excluding the cover pages.
%
Moreover, contents revised in response to the comments of
review 1, 2, and 3 are highlighted in \reviewerA{blue},
\reviewerB{orange}, and \reviewerC{magenta}, respectively.
For updated figures and tables, the captions are colored
similarly to indicate the corresponding reviews.

\newcommand{\qstart}[1]{\vspace{0.15in}\noindent{\bf #1}}
\newcommand{\qother}[1]{\noindent{\bf #1}}
\newcommand{\answer}[1]{\vspace{0.05in}\noindent{\bf #1}}
\newcommand{\feedbk}[1]{\textcolor{darkgray}{\it Feedback: #1}}

\vspace{-0.05in}

\subsection*{1. Review 1}

\vspace{-0.05in}
\qstart{R1.O1}
%
\emph{ It would be useful to specify the tested nprobe parameters in
the experimental setup, and if nprobe can be "safely" lowered for
higher recalls.  Certainly DCO is an intermediary metric), but
understanding how high nprobe is (and potentially how to select it
when we have redundancy) might be helpful for future adopters.  }

\answer{Response:} 
%
In the evaluation, the Recall-QPS and Recall-DCO curves are generated
by varying the $nprobe$ parameter.  Hence, the $nprobe$ setting is not
fixed in the experiments.  

To better understand the impact of $nprobe$ on recalls, we
add a Recall-$nprobe$ figure comparing different solutions in (p.11,
Section~\ref{subsec:overall_perf}, Figure~\ref{fig:nprobe}) and
describe the figure in (p.11, Section~\ref{subsec:overall_perf},
paragraph 2 in Understanding Assignment Strategies with DCO).



\qstart{R1.O2}
%
\emph{ Since this broad category of adding vectors to other partitions
comes with a higher storage footprint, could you clarify the
limitation for in-memory execution. 
%
Initially, this applicability seems unnecessarily limiting, as
technically you only need the codes for fast scan in memory (and
certainly full vectors for rescoring). 
%
Certainly, a discussion about the general applicability of the
approach for disk might make this paper stronger, as nprobe should in
theory be lower.  }

\answer{Response:} 
%
\emph{In-memory footprint}: Our description of SEIL specifically
targets IVFPQ Fast Scan with refine in memory.  As discussed in (p.12,
Section~\ref{subsec:in_depth}, paragraph 3 in Memory Cost), the
additional space cost for RAIRS is 1.2--3.7\%, which is quite
manageable.

\emph{General applicability}: The general idea of exploiting
shared-cells to reduce redundant distance computation and storage
footprint can be applied to different kinds of IVF indices.  For
example, for IVFFlat on disk, which stores IVF lists on disk and
centroids in memory, we can apply the idea of SEIL by replacing the
on-disk lists with shared cells of vectors and recording the
shared cell addresses along with the list centroids in memory.  We add
this discussion on SEIL for IVFFlat on disk in (p.4,
Section~\ref{sec:overview}, last paragraph).

\qstart{R1.O3}
%
\emph{ Regarding nprobe, would you consider providing any guidance on
how to set the parameter to benefit from this redundant assignment?
Is the benefit only from a higher recall or also potentially reduced
nprobe factor which then aims to reduce the query time while improving
recall as well?  }

\answer{Response:} 
%
In (p.11, Section~\ref{subsec:overall_perf}, paragraph 2
in Understanding Assignment Strategies with DCO) in the revision, we
emphasize that the benefit of RAIRS comes not only from higher recalls
but also from lower DCOs, which is evidenced by
Figure~\ref{subfig:redund_dco}.

In the same paragraph, we describe the Recall-$nprobe$ figure (cf.
response to R1.O1).  The findings from the figure can be used to guide
the setting of $nprobe$.
%
Comparing the $nprobe$'s for achieving similar recalls, we see that
the $nprobe$'s of SRAIRS and RAIRS are 42.3\%--46.5\% and
48.1\%--53.1\% of the setting of the baseline single assignment,
respectively.
%
For RAIRS, since a faction of vectors are assigned only once,
achieving recalls comparable to SRAIRS can require a slightly larger
$nprobe$. 


% RAIRS will achieve the highest recalls with the same DCOs.  If one is familar with the nprobe setting of single assignment, then this rule-of-thumb can lead to better recalls with similar query throughput.  

\qstart{R1.O4}
%
\emph{ The claim that RAIRS outperforms SOARL2 should be explained
more in text, as at a first sight some of the differences do not seem
as dramatic (and sometimes seem to be the same).  It is understandable
that sometimes there is a mathematical equivalence between the
distances when these might be close, so explaining why SOARL2 is
indeed sometimes close (and on average also helpful) might be
important for a reader to appreciate the specialization for L2.  }

\answer{Response:} 
%
In the revision, we add in-depth analysis of the results
of SOARL2 in (pp.10-11, Section~\ref{subsec:overall_perf}, Comparison
of Various Assignment Strategies).  
%
Specifically, RAIRS is significantly better than SOARL2 in most cases
because unlike SOAR, RAIRS is optimized for the Euclidean space.  For
SIFT1M at recall 1@1, and SIFT1M and OpenAI at recall 10@10, SOARL2
exhibits performance comparable to RAIRS.
%
AIR prefers to select a $c'$ such that $r'=c'-x$ is closer to the
inverse of $r=c-x$ (i.e., the closer $\theta$ to 180 degrees, the
better).  However, depending on the given data set and the vector in
consideration, the angle $\theta$ for the actual $c'$ may be much
smaller than 180 degrees, resulting in similar assignments as in
SOARL2.
%
Table~\ref{tab:assign_overlap} reports the percentage of vectors whose
2nd-choice centroid under SOARL2 matches the 2nd-choice under AIR.
%
We see that AIR and SOARL2 chooses the same assignment for
72.10\%--95.14\% vectors.  For the above cases where SOARL2 and RAIRS
have similar performance (i.e., SIFT1M and OpenAI), there are high
percentages of 2nd-choice matches.  From another angle, the
4.86\%--27.90\% different assignments lead to the performance benefit
of RAIRS over SOARL2.  Generally, the larger the difference, the
larger the potential benefit of RAIRS. 


\qstart{R1.O5}
%
\emph{ Could you please report recall variance as well, and maybe the
average query latency, p99, p95?  This might highlight better the
impact of your approach.  }

\answer{Response:} 
%
To understand the variance of recalls and query
performance, in the revision, we add a figure to show the CDF
(Cumulative Distribution Function) of recalls and DCOs across all the
10,000 queries for the SIFT1B + 0.95 recall case in (p.11,
Section~\ref{subsec:overall_perf}, Figure~\ref{fig:distribution}) and
describe the figure in (p.11, Section~\ref{subsec:overall_perf},
Distribution of Recalls and DCOs).  
%
From the figure, we see that the recall CDF curves almost overlap, but
RAIRS's DCO curve is clearly to the left of IVFPQfs's DCO curve.  This
means that compared to IVFPQfs, RAIRS significantly reduces the DCOs
for almost all queries while achieving similar recalls.  Moreover, the
recall variance is low; over 89\% of queries achieve 0.8--1.0
recalls.  The p99 DCOs of RAIRS is 1.28x of the average.  The
DCO variance across queries is moderate.  

In addition, we report the query latency for one-query-at-at-time
execution in (p.11, Section~\ref{subsec:overall_perf}, Performance for
One-Query-at-a-Time).  Please see the response to R1.O6/R1.Q1. 

\qstart{R1.O6, R1.Q1}
%
\emph{ If I understand correctly, you are likely running a full query
batch (of 1-10k, depending on the dataset), since you have slightly
different access patterns than just pure IVF is there a penalty if you
run one query at a time, and would you be able to add this discussion
if that seems to be the case (or mention if not).  Are you running
query-at-a-time or a full batch experiments?  }

\answer{Response:} 
%
Yes, we run a full query batch for each experiment by default, which
employs the cache optimization for query batches as described in Sec
5.3.  

In the revision, we add a new experiment to run one query
at a time.  The cache optimization is not used in this experiment.
The experimental results are shown in (p.11,
Section~\ref{subsec:overall_perf}, Figure~\ref{fig:one_query}).  We
describe the results in (p.11, Section~\ref{subsec:overall_perf},
Performance for One-Query-at-a-Time).  We see that RAIRS achieves the
lowest latency among all single assignment and 2-assignment
strategies.  The benefit of RAIRS is similar to that seen in the
batched-query scenarios.


\qstart{R1.M1}
%
\emph{
You could potentially unify how you refer to nprobe (subscript or not).
}

\answer{Response:} 
%
We ensure that $nprobe$ without subscript is used throughout
the paper.  Specifically, we have modified (p.4,
Section~\ref{subsec:air}, paragraph 2 and 3) to use $nprobe$ without
subscript.

\qstart{R1.M2}
%
\emph{
While rescoring can indeed get many more elements than k, 
the example you provide might be slightly exacerbated (Sec 2.2. 10k)
}

\answer{Response:} 
%
As described in Sec 6.1, we use 10 as the default
K\_FACTOR for top-1 and top-10 queries.  Please note that 10 is also a
common setting used for faiss-ivfpqfs experiments in ANN-Benchmark
results~\cite{ANN_Benchmarks}.

To clarify this point, we make the following two changes.  First, in
(p.2, Section~\ref{subsec:ivf}, Refinement), we clarify that $10K$ is
10 multiplied by the top-K parameter.
%
Second, in (p.9, Section~\ref{subsec:exp_setup}, Parameter Setting),
we add the note on the setting used for faiss-ivfpqfs experiments in
ANN-Benchmark results~\cite{ANN_Benchmarks}.


\subsection*{2. Review 2}

\qstart{R2.O1}
%
\emph{ Generalizing SEIL to different block sizes: The current block
size of 32 is heavily influenced by currently available SIMD
instructions.  While performing any experiment within Faiss that
modifies this block size may be infeasible from a practical
perspective, including at least an analytical model, though ideally an
isolated microbenchmark, that explores the interaction between block
size and data would be informative.  }

\answer{Response:} 
%
To understand the impact of block size on SEIL, we vary the block
size, study the change of the number of vectors in shared-blocks and
misc-blocks, and compute the resulting DCOs for a given $nprobe$ in
(p.13, Section~\ref{subsec:in_depth}, Parameter Study for PQ Block
Size).
%
The results show that as the block size increases, there
are more vectors in misc-blocks.  This is expected because the number
of large cells (whose size $\geq$ block size) decreases.  SEIL
performs more redundant distance computation for the vectors in
misc-blocks.


\qstart{R2.O2}
%
\emph{ It is difficult to see the differences between the evaluated
configurations in multiple figures.  In multiple results, the lines
are so close together that it is difficult to draw any conclusion
beyond “our technique is marginally better.” Adding further discussion
that articulates both the figure contents (such as relative
improvements along a specific slice) and the impact of performance
improvements would improve readability.  }

\answer{Response:} 
%
In the revision, to improve readability, we report the
relative improvement of query throughput and DCOs at 0.95 recall in
(p.10, Section~\ref{subsec:overall_perf}, Comparison of Various
Assignment Strategies) and (p.11, Section~\ref{subsec:overall_perf},
Understanding Assignment Strategies with DCO), respectively.  

At 0.95 recall, RAIRS achieves throughput improvement of
1.07–1.33x, 1.11–1.32x, and 1.01–1.23x
compared to IVFPQfs, Na\"iveRA, and SOARL2, respectively.
%
RAIRS reduces the DCO by factors of
0.64–0.83x, 0.62–0.78x, and 0.73–0.99x compared to IVFPQfs,
Na\"iveRA, and SOARL2, respectively.

\qstart{R2.O3}
%
\emph{
Clarification about Intel SIMD instructions
}

\eat{
O3. A. Nit: “AVX256 SIMD” is incorrect terminology. 
The instruction set is named “AVX2”, 
though it includes “256-bit SIMD instructions”. 

O3. B. Clarification: As per Intel’s online specification sheet 
for the experimental machine’s CPU 
(link: https://www.intel.com/content/www/us/en/products/sku/212459/intel-xeon-platinum-8360y-processor-54m-cache-2-40-ghz/specifications.html), 
the Xeon Platinum 8360Y supports both AVX2 and AVX-512, 
though the exact AVX-512 instruction families are not listed. 
The text should note if the CPU does indeed support AVX-512 instructions, 
along with the note that Faiss (currently) does not support AVX-512, 
partially motivated by concerns related to downclocking in prior generations of Intel CPUs 
(see: https://github.com/facebookresearch/faiss/wiki/How-to-make-Faiss-run-faster/\#avx-512-support).

O3. C. Word of Caution: While Faiss does not use AVX-512 intrinsics (by default), 
the Intel MKL might. 
Whether or not the MKL’s possible use of AVX-512 instructions 
will have any meaningful impact on performance is unknown. 
It would be worthwhile to perform a few small tests 
to determine if any license-based downclocking is occurring, 
as this downclocking may disproportionately impact some of the experimental configurations.
}

\answer{Response:} 
%
We look into the downclocking issue and find that downclocking does
not occur in our experiments.

In the revision, we change the description in (p.8,
Section~\ref{subsec:exp_setup}, Machine Configuration). 
%
First, we use the standard terminology ``AVX2'' and ``AVX-512''
instead of ``AVX256''.
%
Second, we add a footnote to clarify that the IndexIVFPQFastScan class
in FAISS v1.8.0 uses AVX2 256-bit SIMD instructions, but the
compilation of FAISS exploits AVX-512 instructions to generate
libfaiss\_avx512.so. 
%
Our experiments use libfaiss\_avx512.so. 
%
In our experiments, downclocking does not occur. 


\qstart{R2.Q1}
%
\emph{ It is unclear if SMT was utilized during the evaluation.  Were
experiments performed that explored the impact of SMT?  }

\answer{Response:} 
%
No, SMT is not used in the evaluation.  We clarify this point in (p.9,
Section~\ref{subsec:exp_setup}, last paragraph of Solutions to
Compare).

\qstart{R2.M1}
%
\emph{ Within Figure 7, the SIFT-1B experiments in 7(a) and 7(b) seem
to have different maximum y-axis values.  Was this a deliberate
choice?  }

\answer{Response:} 
%
Thanks for catching this last-minute graph drawing error!  We redraw
SIFT1B results in (p.10, Section~\ref{subsec:overall_perf},
Figure~\ref{subfig:redund_qps}) to make sure that the
y-axes of the sub-figures are aligned.


\subsection*{3. Review 3}

\qstart{R3.O1, R3.Q1}
%
\emph{
The paper does not evaluate index construction time.
%
What's the cost of index construction?
}

\answer{Response:} 
%
In the revision, we report the construction time including the
training time and insertion time in (p.8,
Section~\ref{subsec:seil_algo}, paragraph 3 in Cost Analysis).
%
In our experiments on SIFT1M, the index construction time is 29.1s and
27.3s for RAIRS and IVFPQfs, respectively. In comparison,
HNSW requires 136.0s for index construction.  Although RAIRS incurs a
6.6\% slowdown relative to IVFPQfs in index construction, it is still
much faster than HNSW.  Consequently, we consider the additional
construction overhead introduced by RAIRS to be within practical
bounds.



\qstart{R3.O2, R3.Q2}
%
\emph{
The paper does not evaluate incremental vector insertion/deletion time.
%
What's the cost for incremental vector update?
}

\answer{Response:} 
%
In the revision, we evaluate vector insertion and deletion.  We make
the following changes.

First, we add the description of the deletion implementation for RAIRS
in (p.9, Section~\ref{subsec:exp_setup}, paragraph 3 in
Implementation).  (The insertion algorithm is shown in
Algorithm~\ref{alg:seil_insert} in p.7.)

Second, we report the experimental results for insertions and
deletions in (p.12, Section~\ref{subsec:overall_perf},
Figure~\ref{fig:insertion_deletion}).  For insertions, we construct
the index with 800,000 vectors, then perform five insertion batches,
each inserting 40,000 new vectors.  For deletions, we build the index
with the full data set, then execute five batches of deletions, each
removing 40,000 vectors.

Third, we discuss the results in (p.12,
Section~\ref{subsec:overall_perf}, Performance of Insertions and
Deletions).
%
Compared to the baseline IVFPQfs, RAIRS's insertion and deletion
throughput is 12.2\% and 4.4\% lower.  This is because
each vector is assigned up to two lists and RAIRS modifies up to twice
as many entries as IVFPQfs.
%
Please note that the ANN search operation is typically much more
frequent than vector insertion and deletion operations.  While
incurring slight extra cost for insertions and deletions, RAIRS
achieves higher ANNS query performance.



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

%The intended scope of our techniques is twofold. RAIR targets redundant-assignment IVF under Euclidean distance, while SEIL extends to redundant-assignment IVF for arbitrary distance metrics. 
%In terms of storage, RAIR can be deployed on any storage medium including disks, whereas SEIL is restricted to in-memory indices because its query procedure entails random address jumps.

